Bagging and Boosting a Treebank Parser

Bagging and boosting, two effective machine learning techniques, are applied to natural language parsing. Experiments using these techniques with a trainable statistical parser are described. The best resulting system provides roughly as large of a gain in F-measure as doubling the corpus size. Error analysis of the result of the boosting technique reveals some inconsistent annotations in the Penn Treebank, suggesting a semi-automatic method for finding inconsistent treebank annotations.

==> boost.stable.fig.tex <==
%auto-ignore 

%\begin{figure}[htbp]
\mbox{
%\begin{tabular}{c}
\begin{tabular}{cccc}
    \epsfig{file=boost.stable.prftrain.eps, width= 0.25\textwidth}
&
    \epsfig{file=boost.stable.prftest.eps, width= 0.25\textwidth}
&
    \epsfig{file=boost.stable.exacttrain.eps, width= 0.25\textwidth}
&
    \epsfig{file=boost.stable.exacttest.eps, width= 0.25\textwidth}
\end{tabular}
}
%\\
%\bigskip

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "varying"
%%% End: 

